Blockchain and radio communications over suborbital spaceflights: Watchtowers and Mystics

The communication between ground and satellites is tough due to long distances and interferences in the propagation medium. Using the blockchain technology and a series of ground nodes, information can be distributed in a secure and reliable way. The satellite discovers nearby ground stations and sends the information that it is verified with other nodes present in the same network. Ground nodes are classified into two types, master (Watchtowers) and working (Mystics) nodes. The Watchtower controls the entering gate of new nodes to the network and the distribution of information between the working nodes.

==> Makefile <==
PAPER_NAME := blockchain-hab

base:
	pdflatex --file-line-error --synctex=1 --shell-escape $(PAPER_NAME).tex 

typewriter:
	lualatex --file-line-error --synctex=1 --shell-escape $(PAPER_NAME).tex

nobib:
	pdflatex --file-line-error --synctex=1 --shell-escape $(PAPER_NAME).tex && \
	pdflatex --file-line-error --synctex=1 --shell-escape $(PAPER_NAME).tex 

all-default-texmf::
	./fix_texmfhome.sh \
	pdflatex --file-line-error --synctex=1 --shell-escape $(PAPER_NAME).tex && \
	bibtex $(PAPER_NAME) && \
	pdflatex --file-line-error --synctex=1 --shell-escape $(PAPER_NAME).tex && \
	pdflatex --file-line-error --synctex=1 --shell-escape $(PAPER_NAME).tex

all:
	pdflatex --file-line-error --synctex=1 --shell-escape $(PAPER_NAME).tex && \
	bibtex $(PAPER_NAME) && \
	pdflatex --file-line-error --synctex=1 --shell-escape $(PAPER_NAME).tex && \
	pdflatex --file-line-error --synctex=1 --shell-escape $(PAPER_NAME).tex

zip: distclean
	pdflatex --file-line-error --synctex=1 --shell-escape $(PAPER_NAME).tex
	bibtex $(PAPER_NAME)
	rm -f *.aux \
	$(PAPER_NAME).log \
	$(PAPER_NAME).blg \
	$(PAPER_NAME).out \
	$(PAPER_NAME).dvi \
	$(PAPER_NAME)*.gz \
	$(PAPER_NAME).zip
	zip -r $(PAPER_NAME).zip . -x '*.git*' '*README.md' '*.sh' '*~*' '*install_elvish_fonts*' '*texmf*' '*.DS_Store*' '*.emacs*' '*.xcf' '*.drawio' '*.pdf'

distclean: clean
	rm -f	$(PAPER_NAME).pdf

clean:
	rm -f *.aux \
	$(PAPER_NAME).log \
	$(PAPER_NAME).blg \
	$(PAPER_NAME).bbl \
	$(PAPER_NAME).out \
	$(PAPER_NAME).dvi \
	$(PAPER_NAME)*.gz \
	$(PAPER_NAME).zip \


install:
	sudo apt-get install texlive-full texlive-luatex texlive-science

